Why is Normalization Necessary for Linear Recommenders?

Despite their simplicity, linear autoencoder (LAE)-based models have shown comparable or even better performance with faster inference speed than neural recommender models. However, LAEs face two critical challenges: (i) popularity bias, which tends to recommend popular items, and (ii) neighborhood bias, which overly focuses on capturing local item correlations. To address these issues, this paper first analyzes the effect of two existing normalization methods for LAEs, i.e., random-walk and symmetric normalization. Our theoretical analysis reveals that normalization highly affects the degree of popularity and neighborhood biases among items. Inspired by this analysis, we propose a versatile normalization solution, called Data-Adaptive Normalization (DAN), which flexibly controls the popularity and neighborhood biases by adjusting item- and user-side normalization to align with unique dataset characteristics. Owing to its model-agnostic property, DAN can be easily applied to various LAE-based models. Experimental results show that DAN-equipped LAEs consistently improve existing LAE-based models across six benchmark datasets, with significant gains of up to 128.57% and 12.36% for long-tail items and unbiased evaluations, respectively. Refer to our code in https://github.com/psm1206/DAN.

==> Tables/tab-norm_toy_examples.tex <==
\begin{figure}
\includegraphics[clip, trim=0cm 0cm 0cm 0cm, width=0.95\columnwidth]{Figures/gram_norm_v5.png} 
\vspace{-3mm}
\caption{A toy example with Sym normalization. } \label{toy_ex}
\vspace{-3mm}
\end{figure}

% It shows the gram matrices and the LAE solution with and without Sym normalization.

==> Tables/tab-session_dataset_statistics.tex <==
\begin{table}[t] \small
\begin{center}
\caption{Statistics of three benchmark datasets used in session-based recommendation. $Gini_{i}$ denotes the Gini index~\cite{ChinCC22} that measures the distribution of interactions within sets of items. User Diversity Index (UDI) means the diversity of users' consumption patterns, in Eq.~\eqref{eq:user_diversity_index}.}
\vspace{-2mm}
\label{tab:session_statistics}
% \begin{tabular}{c|rrrccc}
\begin{tabular}{P{1.5cm}|P{0.9cm}P{0.7cm}|P{0.7cm}P{0.9cm}|P{0.6cm}P{0.6cm}}
\toprule
Dataset     & \#Sessions   & \#Items   & \#Inter.     & Density   & $Gini_{i}$ & UDI \\
\midrule
Diginetica      & 204,532   & 42,862    & 0.78M         & 0.01\%    & 0.55 &  0.62  \\
RetailRocket    & 321,032   & 51,428    & 0.87M         & 0.01\%    & 0.56 &  0.60  \\
Yoochoose       & 470,477   & 19,690    & 1.43M         & 0.02\%    & 0.87 &  0.90  \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-2mm}
\end{table}

% ML-20M      & 136,677   & 20,108    & 10.0M         & 0.36\%    & 0.90 &  0.57  \\
% Netflix     & 463,435   & 17,769    & 56.9M         & 0.69\%    & 0.86 &  0.59  \\
% MSD         & 571,355   & 41,140    & 33.6M         & 0.36\%    & 0.56 &  0.43  \\
% Gowalla     & 29,858    & 40,981    & 1.03M     & 0.01\%    & 0.44 &  0.43 \\
% Yelp2018    & 31,668    & 38,048    & 1.56M     & 0.13\%    & 0.51 &  0.50 \\
% Amazon-book & 52,643    & 91,599    & 2.98M     & 0.06\%    & 0.46 &  0.44 \\


==> Tables/tab-strong-robustness.tex <==
\begin{table} \small % \footnotesize
\caption{Additional performance comparison on six datasets with the strong generalization. `LAE$_\text{DAN}$' indicates LAE equipped with our proposed DAN. The best results are marked in \red{bold}, and the second best results are \blue{underlined}.}
\label{tab:strong_additional_result}
\vspace{-3mm}
\begin{center}
\renewcommand{\arraystretch}{1} % 테이블 행 간격
\begin{tabular}{P{0.3cm}|P{1.1cm}|P{0.7cm}P{0.7cm}|P{0.7cm}P{0.7cm}|P{0.7cm}P{0.7cm}}
\toprule
\multirow{2}{*}{\rotatebox{90}{}} & \multirow{2}{*}{Model}  & \multicolumn{2}{c|}{AOA} & \multicolumn{2}{c|}{Tail}  & \multicolumn{2}{c}{Unbiased} \\
\multirow{11}{*}{\rotatebox{90}{ML-20M}} &  & R@20 & N@20 & R@20 & N@20 & R@20 & N@20 \\ \midrule
& MutlVAE & 0.3895 & 0.3278 & 0.0133 & 0.0077 & 0.2996 & 0.0509 \\
& GF-CF & 0.3250 & 0.2736 & 0.0029 & 0.0022 & 0.2188 & 0.0371 \\ 
& TurboCF & 0.3276 & 0.2728 & 0.0166 & 0.0111 & 0.2336 & 0.0402 \\
& SVD-AE & 0.xxxx & 0.xxxx & 0.xxxx & 0.xxxx & 0.xxxx & 0.xxxx \\ 
& BSPM & 0.3725 & 0.3183 & 0.0104 & 0.0060 & 0.2761 & 0.0463 \\ \cline{2-8}
& LAE$_\text{DAN}$ & 0.3930 & 0.3414 & \red{0.0234} & \red{0.0128} & 0.2925 & \blue{0.0493} \\ 
& EASE$_\text{DAN}$ & \blue{0.3950} & \blue{0.3430} & {0.0217} & {0.0120} & {0.2955} & {0.0497} \\
& RLAE$_\text{DAN}$ & \red{0.3956} & \red{0.3432} & \blue{0.0227} & \blue{0.0127} & \blue{0.2973} & \red{0.0501} \\ \midrule
\multirow{8}{*}{\rotatebox{90}{Yelp2018}}   
& MutlVAE & 0.0963 & 0.0747 & 0.0193 & 0.0121 & 0.0643 & 0.0074 \\
& GF-CF & 0.1134 & 0.0900 & 0.0155 & 0.0078 & 0.0685 & 0.0081 \\ 
& TurboCF & 0.1144 & 0.0930 & 0.0218 & 0.0133 & 0.0735 & 0.0092 \\
& SVD-AE & 0.xxxx & 0.xxxx & 0.xxxx & 0.xxxx & 0.xxxx & 0.xxxx \\ 
& BSPM & 0.1198 & 0.0951 & 0.0251 & 0.0129 & 0.0776 & 0.0090 \\ \cline{2-8}
& LAE$_\text{DAN}$ & {0.1213} & {0.0989} & \blue{0.0305} & \blue{0.0175} & \blue{0.0814} & \blue{0.0099} \\ 
& EASE$_\text{DAN}$ & \blue{0.1215} & \blue{0.0990} & \blue{0.0305} & \blue{0.0175} & \blue{0.0814} & \blue{0.0099} \\ 
& RLAE$_\text{DAN}$ & \red{0.1219} & \red{0.0993} & \red{0.0307} & \red{0.0176} & \red{0.0818} & \red{0.0100} \\ 
\bottomrule
\end{tabular}
% \vspace{-1.5mm}
\end{center}
\end{table}


==> Tables/tab-strong_hyperparameters.tex <==
\begin{table}[t]
\small
\caption{The best hyperparameters of the proposed methods on six datasets with the strong generalization protocol.}
\vspace{-3mm}
\label{tab:best_strong}
\begin{center}
\begin{tabular}{c|c|cccc}
\toprule
Dataset                     & Model         & $\lambda$     & $\alpha$  & $\beta$ & $\xi$ \\ \midrule 
\multirow{3}{*}{ML-20M}     & LAE$_\text{DAN}$       & 0.05          & 0.8         & 0.6     & -\\    
                            & EASE$_\text{DAN}$      & 0.05          & 0.8         & 0.4     & -\\ 
                            & RLAE$_\text{DAN}$      & 0.05          & 0.8         & 0.5     & 0.3 \\ \midrule
\multirow{3}{*}{Netflix}    & LAE$_\text{DAN}$       & 0.05          & 0.9         & 0.5     & -\\    
                            & EASE$_\text{DAN}$      & 0.01          & 0.8         & 0.7     & -\\ 
                            & RLAE$_\text{DAN}$      & 0.01          & 0.8         & 0.7     & 0.1 \\ \midrule
\multirow{3}{*}{MSD}        & LAE$_\text{DAN}$       & 0.05          & 1           & 0.5     & -\\    
                            & EASE$_\text{DAN}$      & 0.05          & 0.9         & 0.5     & -\\ 
                            & RLAE$_\text{DAN}$      & 0.05          & 1           & 0.4     & 0.1 \\ \midrule
\multirow{3}{*}{Gowalla}    & LAE$_\text{DAN}$       & 20            & 0.8         & 0.3     & -\\    
                            & EASE$_\text{DAN}$      & 20            & 0.8         & 0.3     & -\\   
                            & RLAE$_\text{DAN}$      & 20            & 0.8         & 0.3     & 0.1 \\ \midrule
\multirow{3}{*}{Yelp2018}   & LAE$_\text{DAN}$       & 50            & 0.7         & 0.2     & -\\ 
                            & EASE$_\text{DAN}$      & 20            & 0.7         & 0.3     & -\\ 
                            & RLAE$_\text{DAN}$      & 20            & 0.7         & 0.3     & 0.1 \\ \midrule
\multirow{3}{*}{Amazon-book}& LAE$_\text{DAN}$       & 10            & 0.8         & 0.2     & -\\   
                            & EASE$_\text{DAN}$      & 10            & 0.8         & 0.2     & -\\ 
                            & RLAE$_\text{DAN}$      & 10            & 0.8         & 0.2     & 0.3 \\ 
\bottomrule
\end{tabular}
% \vspace{-3mm}
\end{center}
\end{table}


==> Tables/tab-weak_hyperparameters.tex <==
\begin{table}[t]
\small
\caption{The best hyperparameters of the proposed methods on three datasets with the weak generalization protocol.}
\vspace{-3mm}
\label{tab:best_weak}
\begin{center}
\begin{tabular}{c|c|cccc}
\toprule
Dataset                     & Model         & $\lambda$     & $\alpha$       & $\beta$     & $\xi$      \\  \midrule
\multirow{3}{*}{Gowalla}    & LAE$_\text{DAN}$       &  2            &  0.9      &   0.8            &  - \\    
                            & EASE$_\text{DAN}$      &  2            &  0.9      &   0.8            &  - \\   
                            & RLAE$_\text{DAN}$      &  3            &  1      &   0.6            &  0.9 \\ \midrule  
\multirow{3}{*}{Yelp2018}   & LAE$_\text{DAN}$       &   4           &   0.6      &  0.5     & -\\ 
                            & EASE$_\text{DAN}$     & 4           &   0.6      &  0.5     & -\\ 
                            & RLAE$_\text{DAN}$      & 4           &   0.6      &  0.5     & 0.2  \\ \midrule
\multirow{3}{*}{Amazon-book}& LAE$_\text{DAN}$       &   1           &  0.5        &  0.3     & -\\   
                            & EASE$_\text{DAN}$      &   1           &  0.5        &  0.3     & -\\ 
                            & RLAE$_\text{DAN}$      &    1           &  0.5        &  0.3     & 0.1  \\ 
\bottomrule
\end{tabular}
% \vspace{-3mm}
\end{center}
\end{table}
